LLMs can be easily Confused by Instructional Distractions

Despite the fact that large language models (LLMs) show exceptional skill in instruction following tasks, this strength can turn into a vulnerability when the models are required to disregard certain instructions. Instruction-following tasks typically involve a clear task description and input text containing the target data to be processed. However, when the input itself resembles an instruction, confusion may arise, even if there is explicit prompting to distinguish between the task instruction and the input. We refer to this phenomenon as instructional distraction. In this paper, we introduce a novel benchmark, named DIM-Bench, specifically designed to assess LLMs' performance under instructional distraction. The benchmark categorizes real-world instances of instructional distraction and evaluates LLMs across four instruction tasks: rewriting, proofreading, translation, and style transfer -- alongside five input tasks: reasoning, code generation, mathematical reasoning, bias detection, and question answering. Our experimental results reveal that even the most advanced LLMs are susceptible to instructional distraction, often failing to accurately follow user intent in such cases.

==> rsc/Table_main.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{0.8\textwidth}{!}{% 
\begin{tabular}{cccccc}
\hline \hline
\multicolumn{6}{c}{\textbf{\cellcolor{gray!10}\textit{LLAMA 3.1 8B Inst.}}}                                                                                               \\ \hline 
\multicolumn{1}{c|}{\diagbox[height=0.85cm]{\textit{Instruction}}{\textit{Input}}}              & \multicolumn{1}{c}{\phantom{00}\textbf{Reasoning}\phantom{00}} & \textbf{Code Generation} &\phantom{00} \textbf{Math}\phantom{00} & \textbf{Bias Detection} & \textbf{Question Answering} \\ \hline
\multicolumn{1}{c|}{\textbf{Rewriting}}       & 0.15                     & 0.89            & 0.43      & 0.01           & 0.09               \\ \hline
\multicolumn{1}{c|}{\textbf{Proofreading}}     & 0.68                     & 0.86            & 0.83      & 0.52           & 0.00               \\ \hline
\multicolumn{1}{c|}{\textbf{Translation}}   & 0.54                     & 0.61            & 0.83      & 0.22           & 0.18               \\ \hline
\multicolumn{1}{c|}{\textbf{Style Transfer}} & 0.06                     & 0.16            & 0.46      & 0.02           & 0.02               \\ \hline
\multicolumn{6}{c}{\textbf{\cellcolor{gray!10}\textit{LLAMA 3.1 70B Inst.}}}                                                                                          \\ \hline
\multicolumn{1}{c|}{\diagbox[height=0.85cm]{\textit{Instruction}}{\textit{Input}}}              & \multicolumn{1}{c}{\phantom{00} \textbf{Reasoning}\phantom{00}} & \textbf{Code Generation} & \textbf{Math} & \textbf{Bias Detection} & \textbf{Question Answering} \\ \hline
\multicolumn{1}{c|}{\textbf{Rewriting}}       & 0.15                     & 0.85            & 0.81      & 0.15           & 0.00               \\ \hline
\multicolumn{1}{c|}{\textbf{Proofreading}}     & 0.70                     & 0.87            & 0.91      & 0.82           & 0.00               \\ \hline
\multicolumn{1}{c|}{\textbf{Translation}}   & 0.75                     & 0.82            & 0.96      & 0.44           & 0.10               \\ \hline
\multicolumn{1}{c|}{\textbf{Style Transfer}} & 0.26                     & 0.31            & 0.63      & 0.31           & 0.00               \\ \hline
\multicolumn{6}{c}{\textbf{\cellcolor{gray!10}\textit{GPT-3.5}}}                                                                                          \\ \hline
\multicolumn{1}{c|}{\diagbox[height=0.85cm]{\textit{Instruction}}{\textit{Input}}}              & \multicolumn{1}{c}{\phantom{00} \textbf{Reasoning}\phantom{00}} & \textbf{Code Generation} & \textbf{Math} & \textbf{Bias Detection} & \textbf{Question Answering} \\ \hline
\multicolumn{1}{c|}{\textbf{Rewriting}}       & 0.15                     & 0.78            & 0.68      & 0.03           & 0.09               \\ \hline
\multicolumn{1}{c|}{\textbf{Proofreading}}     & 0.51                     & 0.86            & 0.86      & 0.26           & 0.04               \\ \hline
\multicolumn{1}{c|}{\textbf{Translation}}   & 0.51                     & 0.79            & 0.87      & 0.08           & 0.42               \\ \hline
\multicolumn{1}{c|}{\textbf{Style Transfer}} & 0.39                     & 0.49            & 0.51      & 0.03           & 0.22               \\ \hline
\multicolumn{6}{c}{\textbf{\cellcolor{gray!10}\textit{GPT-4o-mini}}}                                                                                \\ \hline
\multicolumn{1}{c|}{\diagbox[height=0.85cm]{\textit{Instruction}}{\textit{Input}}}              & \multicolumn{1}{c}{\phantom{00} \textbf{Reasoning}\phantom{00}} & \textbf{Code Generation} & \textbf{Math} & \textbf{Bias Detection} & \textbf{Question Answering} \\ \hline
\multicolumn{1}{c|}{\textbf{Rewriting}}       & 0.57                     & 0.93            & 0.95      & 0.32           & 0.02               \\ \hline
\multicolumn{1}{c|}{\textbf{Proofreading}}     & 0.72                     & 0.68            & 0.98      & 0.60           & 0.00               \\ \hline
\multicolumn{1}{c|}{\textbf{Translation}}   & 0.75                     & 0.83            & 0.96      & 0.47           & 0.36               \\ \hline
\multicolumn{1}{c|}{\textbf{Style Transfer}} & 0.61                     & 0.50            & 0.67      & 0.07           & 0.32               \\ \hline
\multicolumn{6}{c}{\textbf{\cellcolor{gray!10}\textit{GPT-4o}}}                                                                               \\ \hline
\multicolumn{1}{c|}{\diagbox[height=0.85cm]{\textit{Instruction}}{\textit{Input}}}              & \multicolumn{1}{c}{\phantom{00} \textbf{Reasoning}\phantom{00}} & \textbf{Code Generation} & \textbf{Math} & \textbf{Bias Detection} & \textbf{Question Answering} \\ \hline
\multicolumn{1}{c|}{\textbf{Rewriting}}       & 0.50                     & 0.89            & 0.93      & 0.11           & 0.00               \\ \hline
\multicolumn{1}{c|}{\textbf{Proofreading}}     & 0.84                     & 0.47            & 0.98      & 0.52           & 0.00               \\ \hline
\multicolumn{1}{c|}{\textbf{Translation}}   & 0.72                     & 0.83            & 0.96      & 0.26           & 0.15               \\ \hline
\multicolumn{1}{c|}{\textbf{Style Transfer}} & 0.47                     & 0.53            & 0.57      & 0.08           & 0.04               \\ \hline \hline
\end{tabular}
 }
\caption{The results of instruction-following performance under instruction distraction for five different LLMs measured using DIM-Bench. The values represent accuracy.}
\label{table_main_old}
\vspace{-5mm}
\end{table*}

